Perturbing Inputs for Fragile Interpretations in Deep Natural Language Processing

Interpretability methods like Integrated Gradient and LIME are popular choices for explaining natural language model predictions with relative word importance scores. These interpretations need to be robust for trustworthy NLP applications in high-stake areas like medicine or finance. Our paper demonstrates how interpretations can be manipulated by making simple word perturbations on an input text. Via a small portion of word-level swaps, these adversarial perturbations aim to make the resulting text semantically and spatially similar to its seed input (therefore sharing similar interpretations). Simultaneously, the generated examples achieve the same prediction label as the seed yet are given a substantially different explanation by the interpretation methods. Our experiments generate fragile interpretations to attack two SOTA interpretation methods, across three popular Transformer models and on two different NLP datasets. We observe that the rank order correlation drops by over 20% when less than 10% of words are perturbed on average. Further, rank-order correlation keeps decreasing as more words get perturbed. Furthermore, we demonstrate that candidates generated from our method have good quality metrics.

==> 061-table-more.tex <==
\begin{table*}[]
\centering
% \resizebox{\textwidth}{}
% \begin{adjustbox}{width=\textwidth,center}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{ccccccc|cccccc}
\hline
& \multicolumn{6}{c}{SST-2} & \multicolumn{6}{c}{AGNews} \\
\hline
& \multicolumn{2}{c}{DistilBERT} & \multicolumn{2}{c}{RoBERTa} & \multicolumn{2}{c}{BERT-adv} & \multicolumn{2}{c}{DistilBERT} & \multicolumn{2}{c}{RoBERTa} & \multicolumn{2}{c}{BERT-adv} \\
\hline
Ratio & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM \\
\hline
0-0.1 & 0.72 & 0.77 & 0.8 & 0.82 & 0.76 & 0.73 & 0.87 & 0.84 & 0.61 & 0.6 & 0.77 & 0.75 \\
0.1-0.2 & 0.66 & 0.7 & 0.73 & 0.73 & 0.68 & 0.65 & 0.74 & 0.79 & 0.54 & 0.5 & 0.69 & 0.69 \\
0.2-0.3 & 0.69 & 0.67 & 0.69 & 0.7 & 0.64 & 0.63 & 0.66 & 0.75 & 0.51 & 0.48 & 0.64 & 0.63 \\
0.3-0.4 & 0.7 & 0.68 & 0.68 & 0.64 & 0.71 & 0.67 & 0.6 & 0.73 & 0.52 & 0.46 & 0.61 & 0.59 \\
0.4-0.5 & 0.65 & 0.67 & 0.64 & 0.61 & 0.7 & 0.65 & 0.61 & 0.72 & 0.44 & 0.44 & 0.59 & 0.57 \\
\hline
\end{tabular}%
}
% \end{adjustbox}
\caption{Change in average Top-50\% intersection using metrics - \diffs and \nobjs conmputed using the interpretability method: \victimI, across 2 datasets- SST-2 and AG News over 3 models - DistilBERT, RoBERTa and BERT-adv.}
\label{tab:IG-TopK}
\end{table*}





\begin{table*}[]
\centering
% \resizebox{\textwidth}{}
% \begin{adjustbox}{width=\textwidth,center}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{ccccccc|cccccc}
\hline
& \multicolumn{6}{c}{SST-2} & \multicolumn{6}{c}{AGNews} \\
\hline
& \multicolumn{2}{c}{DistilBERT} & \multicolumn{2}{c}{RoBERTa} & \multicolumn{2}{c}{BERT-adv} & \multicolumn{2}{c}{DistilBERT} & \multicolumn{2}{c}{RoBERTa} & \multicolumn{2}{c}{BERT-adv} \\
\hline
& L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM \\
\hline
0-0.1 & 0.41 & 0.37 & 0.67 & 0.73 & 0.67 & 0.68 & 0.75 & 0.58 & 0.56 & 0.44 & 0.58 & 0.59\\
0.1-0.2 & 0.38 & 0.35 & 0.61 & 0.72 & 0.63 & 0.62 & 0.66 & 0.48 & 0.46 & 0.44 & 0.56 & 0.56 \\
0.2-0.3 & 0.39 & 0.35 & 0.6 & 0.67 & 0.6 & 0.6 & 0.56 & 0.36 & 0.44 & 0.42 & 0.54 & 0.53 \\
0.3-0.4 & 0.37 & 0.33 & 0.68 & 0.65 & 0.59 & 0.58 & 0.51 & 0.36 & 0.43 & 0.42 & 0.50 & 0.50 \\
0.4-0.5 & 0.33 & 0.27 & 0.66 & 0.66 & 0.6 & 0.6 & 0.45 & 0.36 & 0.43 & 0.41 & 0.49 & 0.44 \\
\hline
\end{tabular}%
}
% \end{adjustbox}
\caption{Change in average Top-50\% intersection using metrics - \diffs and \nobjs conmputed using the interpretability method: \victimL, across 2 datasets- SST-2 and AG News over 3 models - DistilBERT, RoBERTa and BERT-adv.}
\label{tab:LIME-TopK}
\end{table*}

\begin{table}[t]
\centering
% \resizebox{\textwidth}{}
% \begin{adjustbox}{width=\textwidth,center}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
& \multicolumn{6}{c}{IMDB} \\
\hline
& \multicolumn{2}{c}{DistilBERT} & \multicolumn{2}{c}{RoBERTa} & \multicolumn{2}{c}{BERT-adv} \\
\hline
Ratio & L2 & $\Delta$LOM & L2 & $\Delta$LOM & L2 & $\Delta$LOM \\
\hline
0-0.1 & 0.69 & 0.69 & 0.75 & 0.74 & 0.45 & 0.44 \\
0.1-0.2 & 0.53 & 0.55 & 0.64 & 0.59 & 0.32 & 0.32 \\
0.2-0.3 & 0.41 & 0.44 & 0.51 & 0.48 & 0.28 & 0.29 \\
0.3-0.4 & 0.42 & 0.39 & 0.45 & 0.41 & 0.27 & 0.28 \\
0.4-0.5 & 0.33 & 0.31 & 0.34 & 0.37 & 0.12 & 0.17 \\
\hline
\end{tabular}
}
\caption{Change in average Rank Correlation using metrics - \diffs and \nobjs conmputed using the interpretability method: \victimI, across dataset- IMDB over 3 models - DistilBERT, RoBERTa and BERT-adv.}
\label{tab:IG-Rank-IMDB}
\vspace{-5mm}
\end{table}


==> 062-baseline.tex <==
% \qnote{I feel another issue of your paper is the lack of a baseline..
% 7:33
% can you just try randomly perturb at the same ratio of words..
% 7:34
% and show how the resulting interpretation vary from the original..
% 7:34
% is this possible…
% 7:34
% at least one one dataset… one model…
% 7:34
% this can provide a solid table showing… your method is much more effective than the random baseline…}

==> 063-results2Appx.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multicolumn{10}{c}{AGNews} \\
\hline
& \multicolumn{3}{c}{DistilBERT} & \multicolumn{3}{c}{RoBERTa} & \multicolumn{3}{c}{BERT-adv} \\
\hline
Ratio & L2 & LOM & Random & L2 & LOM & Random & L2 & LOM & Random \\
\hline
0-0.1 & 0.81 & 0.84 & 0.86 & 0.73 & 0.68 & 0.82 & 0.38 & 0.56 & 0.63 \\
0.1-0.2 & 0.72 & 0.75 & 0.78 & 0.65 & 0.57 & 0.72 & 0.32 & 0.42 & 0.46 \\
0.2-0.3 & 0.64 & 0.66 & 0.69 & 0.62 & 0.52 & 0.66 & 0.28 & 0.32 & 0.29 \\
0.3-0.4 & 0.55 & 0.58 & 0.58 & 0.58 & 0.48 & 0.62 & 0.25 & 0.25 & 0.26 \\
0.4-0.5 & 0.49 & 0.52 & 0.56 & 0.52 & 0.42 & 0.56 & 0.18 & 0.23 & 0.24 \\
\hline
\end{tabular}
}
\caption{Change in average rank-order correlation using metrics - \diffs, \nobjs and random selection conmputed using the interpretability method: \victimI, for dataset- AGNews over 3 models - DistilBERT, RoBERTa and BERT-adv. \label{tab:agnews-IG-rank}
}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multicolumn{10}{c}{AGNews} \\
\hline
& \multicolumn{3}{c}{DistilBERT} & \multicolumn{3}{c}{RoBERTa} & \multicolumn{3}{c}{BERT-adv} \\
\hline
Ratio & L2 & LOM & Random & L2 & LOM & Random & L2 & LOM & Random \\
\hline
0-0.1 & 0.64 & 0.65 & 0.71 & 0.7 & 0.74 & 0.85 & 0.48 & 0.51 & 0.79 \\
0.1-0.2 & 0.57 & 0.58 & 0.69 & 0.61 & 0.64 & 0.8 & 0.37 & 0.4 & 0.69 \\
0.2-0.3 & 0.57 & 0.58 & 0.62 & 0.55 & 0.59 & 0.77 & 0.24 & 0.27 & 0.64 \\
0.3-0.4 & 0.53 & 0.53 & 0.58 & 0.52 & 0.55 & 0.74 & 0.22 & 0.24 & 0.6 \\
0.4-0.5 & 0.51 & 0.52 & 0.56 & 0.45 & 0.5 & 0.71 & 0.19 & 0.24 & 0.58 \\
\hline
\end{tabular}

}
\caption{Change in average Top-50\% intersection using metrics - \diffs, \nobjs and random selection conmputed using the interpretability method: \victimI, for dataset- AGNews over 3 models - DistilBERT, RoBERTa and BERT-adv. \label{tab:agnews-IG-topk}}

\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multicolumn{10}{c}{AGNews} \\
\hline
& \multicolumn{3}{c}{DistilBERT} & \multicolumn{3}{c}{RoBERTa} & \multicolumn{3}{c}{BERT-adv} \\
\hline
Ratio & L2 & LOM & Random & L2 & LOM & Random & L2 & LOM & Random \\
\hline
0-0.1 & 0.65 & 0.69 & 0.71 & 0.58 & 0.57 & 0.61 & 0.7 & 0.61 & 0.72 \\
0.1-0.2 & 0.59 & 0.6 & 0.62 & 0.55 & 0.54 & 0.56 & 0.69 & 0.45 & 0.7 \\
0.2-0.3 & 0.53 & 0.53 & 0.58 & 0.54 & 0.53 & 0.48 & 0.65 & 0.35 & 0.66 \\
0.3-0.4 & 0.48 & 0.52 & 0.55 & 0.51 & 0.51 & 0.36 & 0.65 & 0.28 & 0.65 \\
0.4-0.5 & 0.44 & 0.38 & 0.46 & 0.43 & 0.42 & 0.43 & 0.59 & 0.26 & 0.61 \\
\hline
\end{tabular}
}
\caption{Change in average rank-order correlation using metrics - \diffs, \nobjs and random selection conmputed using the interpretability method: \victimL, for dataset- AGNews over 3 models - DistilBERT, RoBERTa and BERT-adv. \label{tab:agnews-LIME-rank}}

\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multicolumn{10}{c}{AGNews} \\
\hline
& \multicolumn{3}{c}{DistilBERT} & \multicolumn{3}{c}{RoBERTa} & \multicolumn{3}{c}{BERT-adv} \\
\hline
Ratio & L2 & LOM & Random & L2 & LOM & Random & L2 & LOM & Random \\
\hline
0-0.1 & 0.62 & 0.64 & 0.66 & 0.6 & 0.62 & 0.61 & 0.56 & 0.56 & 0.55 \\
0.1-0.2 & 0.58 & 0.59 & 0.63 & 0.58 & 0.58 & 0.58 & 0.53 & 0.54 & 0.53 \\
0.2-0.3 & 0.57 & 0.57 & 0.58 & 0.55 & 0.57 & 0.57 & 0.51 & 0.51 & 0.52 \\
0.3-0.4 & 0.55 & 0.56 & 0.58 & 0.55 & 0.55 & 0.57 & 0.5 & 0.5 & 0.52 \\
0.4-0.5 & 0.53 & 0.55 & 0.57 & 0.54 & 0.54 & 0.56 & 0.51 & 0.5 & 0.52 \\
\hline
\end{tabular}
}
\caption{Change in average Top-50\% intersection using metrics - \diffs, \nobjs and random selection conmputed using the interpretability method: \victimL, for dataset- AGNews over 3 models - DistilBERT, RoBERTa and BERT-adv. \label{tab:agnews-LIME-topk}}
% \vspace{-5mm}
\end{table*}



\begin{figure}[thb]
    \centering
     \includegraphics[width=0.48\textwidth]{images/ablation-sst2.pdf} 
        \caption{The violin graphs demonstrate the effectiveness of candidate selection based on the proposed metrics \nobjs and \diffs over random selection. As it can be seen that the selection based on the proposed metrics disrupts rank correlation more as compared to randomly selecting candidates.
          \label{fig:ablation-sst2} }
\end{figure}


\begin{figure*}[!ht]
\centering 
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violincom-sst2-distilbert-last.png}
    \endminipage\hfill
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violincom-sst2-roberta-last.png} 
    \endminipage\hfill
    \minipage{0.34\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violionplot-bert-sst2-lom.png} 
    \endminipage\hfill
    \caption{Average Rank-correlation for the dataset: SST-2, using metric: \nobjs on models DistilBERT, RoBERTa and BERT-adv using interpretability method -\victimI }
    \label{fig:violinplots-sst-ig-lom}
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violionplot-lime-sst-distil.png} 
    \endminipage\hfill
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violionplot-lime-sst-roberta.png} 
    \endminipage\hfill
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violinplot-sst2-bert-adv-lime.png} 
    \endminipage\hfill
    \caption{Average Rank-correlation for the dataset: SST-2, using metric: \nobjs on models DistilBERT, RoBERTa and BERT-adv using interpretability method -\victimL }
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violionplot-distilbert-sst2-l2-newest.png}
    \endminipage\hfill
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violionplot-roberta-sst2-l2-newest.png} 
    \endminipage\hfill
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violionplot-bert-sst2-l2.png} 
    \endminipage\hfill
    \caption{Average Rank-correlation for the dataset: SST-2, using metric: \diffs on models DistilBERT, RoBERTa and BERT-adv using interpretability method -\victimI }
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violinplot-sst2-distilbert-lime-l2.png} 
    \endminipage\hfill
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violinplot-sst2-roberta-lime-l2.png} 
    \endminipage\hfill
    \minipage{0.33\textwidth}
     \includegraphics[width=\textwidth]{images/violins/SST2/violionplot-lime-sst-bert-adv.png}
    \endminipage\hfill
    \caption{Average Rank-correlation for the dataset: SST-2, using metric: \diffs on models DistilBERT, RoBERTa and BERT-adv using interpretability method -\victimL }
    \label{fig:violinplots-sst-lime-l2}
\end{figure*}


%%%%%%%
\iffalse 




\begin{figure*}[!ht]
\centering 
    \begin{minipage}[t]{0.75\hsize} 
     \includegraphics[width=\textwidth]{images/violin-ig-distilbert.pdf} 
     \label{fig:violin-distil-ig}
    \end{minipage} 
    \begin{minipage}[t]{0.75\hsize} 
     \includegraphics[width=\textwidth]{images/violin-ig-roberta.pdf} 
     \label{fig:violin-roberta-ig}
    \end{minipage} 
    \caption{The Violin plots demonstrate the change in Rank Order Correlation vs Ratio of words perturbed on the (a) SST-2 dataset (Top-Left) (b) AG-News Dataset (Top-Right) and (c) IMDB dataset (Bottom) on the models DistilBERT-uncased (top) and RoBERTa (bottom) - (d), (e) and (f) respectively for SST-2, AG News and IMDB. \qnote{the layout of these sub figures look quite bad..I think we should use them as showing ablation analysis.. each subfigure should include another curve showing the ablated baseline like selecting random position to perturb.... that will make the message much stronger..} }
    \label{fig:table-violin-ig} 
\end{figure*}



\subsection{More empirical results}

\begin{figure*}[!ht]
\centering 
%     \begin{minipage}[t]{0.99\hsize} 
%       \centering 
%       \begin{tabularx}{\textwidth}{|c|c|c|c|c|}
% \hline
% \textbf{Model}                       & \multicolumn{1}{c|}{\textbf{Dataset}} & \textbf{SST-2} & \textbf{AG NEWS} & \textbf{IMDB}                           \\ \hline
% \multirow{5}{*}{\textbf{DistilBERT}} & \textless{}0.1                        & 0.70 +/- 0.18  & 0.69 +/- 0.14    & \multirow{10}{*}{Exponential Time} \\ \cline{2-4}
%                                      & 0.1-0.2                               & 0.58 +/- 0.21  & 0.60 +/- 0.19    &                                         \\ \cline{2-4}
%                                      & 0.2-0.3                               & 0.51 +/- 0.20  & 0.53 +/- 0.19    &                                         \\ \cline{2-4}
%                                      & 0.3-0.4                               & 0.43 +/- 0.21  & 0.52 +/- 0.15    &                                         \\ \cline{2-4}
%                                      & 0.4-0.5                               & 0.29 +/- 0.24  & 0.38 +/- 0.14    &                                         \\ \cline{1-4}
% \multirow{5}{*}{\textbf{RoBERTa}}    & \textless{}0.1                        & 0.66 +/- 0.20  & 0.57 +/- 0.15    &                                         \\ \cline{2-4}
%                                      & 0.1-0.2                               & 0.63 +/- 0.18  & 0.54 +/- 0.15    &                                         \\ \cline{2-4}
%                                      & 0.2-0.3                               & 0.58 +/- 0.18  & 0.53 +/- 0.14    &                                         \\ \cline{2-4}
%                                      & 0.3-0.4                               & 0.54 +/- 0.20  & 0.51 +/- 0.15    &                                         \\ \cline{2-4}
%                                      & 0.4-0.5                               & 0.55 +/- 0.15  & 0.42 +/- 0.13    &                                         \\ \hline
% \end{tabularx}
% \caption{\\The table demonstrates the change in rank-order correlation using the method: \victimL over 3 datasets: SST-2, AG News, IMDB and 2 models: DistilBERT and RoBERTa}
%     \end{minipage} \hfill
    \begin{minipage}[t]{0.9\hsize} 
     \includegraphics[width=\textwidth]{images/violin-distil-lime.pdf} 
    \end{minipage} 
    \begin{minipage}[t]{0.9\hsize} 
     \includegraphics[width=\textwidth]{images/violin-roberta-lime.pdf} 
    \end{minipage} 
    \caption{The Violin plots demonstrate the change in Rank Order Correlation vs Ratio of words perturbed on the (a) SST-2 dataset (Left) (b) AG-News Dataset (Right) on the models DistilBERT-uncased (top) and RoBERTa (bottom) - (c) and (d) respectively for SST-2 and AG News. 
          \label{fig:table-violin-lime} \qnote{I think we should use them as showing ablation analysis.. each subfigure should include another curve showing the ablated baseline like selecting random position to perturb.... that will make the message much stronger.. }}
\end{figure*}



% \begin{figure*}[thb]
%     \centering
%      \includegraphics[width=0.79\textwidth]{images/examplesroberta.pdf} 
%         \caption{The figure demonstrates some examples on RoBERTa model/SST-2 [Best viewed in color]
%           \label{fig:exroberta} }
% \end{figure*}






\begin{figure*}[!ht]
\centering 
    % \begin{minipage}[t]{0.90\hsize} 
    %   \centering 
    %   \begin{tabularx}{\textwidth}{|c|c|c|c|c|}
    %     \hline
    % \textbf{Model}                       & \textbf{Dataset}        & \textbf{SST-2}         & \textbf{AG NEWS}       & \textbf{IMDB}          \\ \hline
    % \multirow{5}{*}{\textbf{DistilBERT}} & \textless{}0.1 & 0.78 +/- 0.31 & 0.84 +/- 0.11 & 0.69 +/- 0.16 \\ \cline{2-5} 
    %                         & 0.1-0.2        & 0.65 +/-0.32  & 0.75 +/- 0.13 & 0.55 +/- 0.13 \\ \cline{2-5} 
    %                         & 0.2-0.3        & 0.55 +/- 0.28 & 0.66 +/- 0.14 & 0.44 +/- 0.12 \\ \cline{2-5} 
    %                         & 0.3-0.4        & 0.48 +/- 0.27 & 0.58 +/- 0.15 & 0.39 +/- 0.12 \\ \cline{2-5} 
    %                         & 0.4-0.5        & 0.42 +/- 0.28 & 0.52 +/- 0.17 & 0.31 +/- 0.15 \\ \hline
    % \multirow{5}{*}{\textbf{RoBERTa}}    & \textless{}0.1 & 0.84 +/- 0.22 & 0.68 +/- 0.22 & 0.62 +/- 0.15 \\ \cline{2-5} 
    %                         & 0.1-0.2        & 0.75 +/- 0.22 & 0.57 +/- 0.21 & 0.49 +/- 0.12 \\ \cline{2-5} 
    %                         & 0.2-0.3        & 0.66 +/- 0.21 & 0.52 +/- 0.21 & 0.39 +/- 0.11 \\ \cline{2-5} 
    %                         & 0.3-0.4        & 0.58 +/- 0.21 & 0.48 +/- 0.20 & 0.35 +/- 0.11 \\ \cline{2-5} 
    %                         & 0.4-0.5        & 0.51 +/- 0.21 & 0.42 +/- 0.21 & 0.28 +/- 0.15 \\ \hline
    % \end{tabularx}
    % \caption{The table demonstrates the change in rank-order correlation using the method: \victimI over 3 datasets: SST-2, AG News, IMDB and 2 models: DistilBERT and RoBERTa}
    % \end{minipage} \hfill
    \begin{minipage}[t]{0.75\hsize} 
     \includegraphics[width=\textwidth]{images/violin-ig-distilbert.pdf} 
     \label{fig:violin-distil-ig}
    \end{minipage} 
    \begin{minipage}[t]{0.75\hsize} 
     \includegraphics[width=\textwidth]{images/violin-ig-roberta.pdf} 
     \label{fig:violin-roberta-ig}
    \end{minipage} 
    \caption{The Violin plots demonstrate the change in Rank Order Correlation vs Ratio of words perturbed on the (a) SST-2 dataset (Top-Left) (b) AG-News Dataset (Top-Right) and (c) IMDB dataset (Bottom) on the models DistilBERT-uncased (top) and RoBERTa (bottom) - (d), (e) and (f) respectively for SST-2, AG News and IMDB. \qnote{the layout of these sub figures look quite bad..I think we should use them as showing ablation analysis.. each subfigure should include another curve showing the ablated baseline like selecting random position to perturb.... that will make the message much stronger..} }
    \label{fig:table-violin-ig} 
\end{figure*}






\fi 


==> 08-ethics.tex <==
\section{Ethics Statement}



